Near-chip Dynamic Vision Filtering for Low-Bandwidth Pedestrian Detection

This paper presents a novel end-to-end system for pedestrian detection using Dynamic Vision Sensors (DVSs). We target applications where multiple sensors transmit data to a local processing unit, which executes a detection algorithm. Our system is composed of (i) a near-chip event filter that compresses and denoises the event stream from the DVS, and (ii) a Binary Neural Network (BNN) detection module that runs on a low-computation edge computing device (in our case a STM32F4 microcontroller). We present the system architecture and provide an end-to-end implementation for pedestrian detection in an office environment. Our implementation reduces transmission size by up to 99.6% compared to transmitting the raw event stream. The average packet size in our system is only 1397 bits, while 307.2 kb are required to send an uncompressed DVS time window. Our detector is able to perform a detection every 450 ms, with an overall testing F1 score of 83%. The low bandwidth and energy properties of our system make it ideal for IoT applications.

==> Makefile <==
# @fclad
# Simple makefile to compile paper with latexmk. Change DIR_OUTPUT for
# a tmpfs path, you really don't want to use your write cycles of your
# SSD compiling a paper

NAME = isvlsi_dvs
LATEX = latexmk -pdf -bibtex -pvc -jobname=$(NAME)
DIR_OUTPUT = /tmp/Volatile

## Sources
SRC = $(NAME).tex

.PHONY	: all clean \
          essay

all 	: essay

essay 	:
	$(LATEX) $(SRC) > /dev/null

# @fclad
# A better clean is rm -rf / but that may have unintended consequences
clean	:
	@-rm -f $(DIR_OUTPUT)/$(NAME)*

